G-HOP: Generative Hand-Object Prior for Interaction Reconstruction and Grasp Synthesis

We propose G-HOP, a denoising diffusion based generative prior for hand-object interactions that allows modeling both the 3D object and a human hand, conditioned on the object category. To learn a 3D spatial diffusion model that can capture this joint distribution, we represent the human hand via a skeletal distance field to obtain a representation aligned with the (latent) signed distance field for the object. We show that this hand-object prior can then serve as generic guidance to facilitate other tasks like reconstruction from interaction clip and human grasp synthesis. We believe that our model, trained by aggregating seven diverse real-world interaction datasets spanning across 155 categories, represents a first approach that allows jointly generating both hand and object. Our empirical evaluations demonstrate the benefit of this joint prior in video-based reconstruction and human grasp synthesis, outperforming current task-specific baselines. Project website: https://judyye.github.io/ghop-www

==> fig/fig_userstudy.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/user_study_3DW.pdf}
    \caption{{\textbf{User study of Human Grasp Synthesis: } } We show preference percentages from users for each pairwise method comparison on HO3D and ObMAN. }
    \label{fig:enter-label}
\end{figure}

==> fig/improve.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{example-image-duck}
    \caption{\textbf{Improving Single-View Reconstruction:} Image | off-the-shelf prediction (from 2 views) | SDS (from same 2 views) }
    \label{fig:enter-label}
\end{figure}

==> table/grasp_2col.tex <==

\begin{figure*}[ht]
    \centering
    % Adjust the widths of the minipages to fit side by side
    \begin{minipage}[b]{0.48\linewidth}
        \centering
        % Resize the table to fit within the minipage
\resizebox{\linewidth}{!}{
\begin{tabular}{l c c c c c c c c c }
\toprule

% CATEGORIES
&
& \multicolumn{3}{c}{Intersection} 
& \multicolumn{1}{c}{Disp.}
& \multicolumn{2}{c}{Contact}
\\
% RULES
\cmidrule(lr){3-5} \cmidrule(lr){6-6} \cmidrule(lr){7-8}

& & maxD$\downarrow$  & avgD$\downarrow$ & vol$\downarrow$ & avg $\downarrow$  & ratio$\uparrow$ & area$\uparrow$ \\
\midrule
\multirow{3}{*}{HO3D} 
& GT &  \textbf{1.32} &  0.37 &  6.16 &  2.32 & 0.95 & 0.15 \\
& GraspTTA & 2.44 & 0.61 &  \textbf{5.25} & 2.89 &  1.00 &  0.23 \\
& \ours &  1.84 &  \textbf{0.31} & 11.46 &  \textbf{0.95} &  \textbf{1.00} &  \textbf{0.23} \\

\midrule

\multirow{3}{*}{ObMan} 
& GT & 0.98 & 0.74 &  \textbf{1.70} &  1.57 &  1.00 & 0.12 \\
& GraspTTA &  0.87 &  0.58 &  5.56 &  \textbf{1.54} &  \textbf{1.00} &  0.18 \\
& \ours &  \textbf{0.74} &  \textbf{0.51} & 17.40 & 1.85 & 0.93 &  \textbf{0.25} \\


\bottomrule
\end{tabular}
}

        \captionof{table}{\textbf{Comparison with Baselines:} We compare human grasp synthesis along with prior work~\cite{jiang2021hand} and annotated grasps provided by datasets(GT) on HO3D and ObMan. We report in table the amount of intersection between meshes, displacement distance in simulation, and hand contact ratio and area.  }
        \label{tab:grasp}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.48\linewidth}
        \centering
        % Adjust the size of the figure to match the table's height
        \includegraphics[width=\linewidth,height=\dimexpr \textheight - 2\baselineskip\relax,keepaspectratio]{fig/userstudy.pdf}
        % Separate caption for the figure
        \caption{{\textbf{User study of Human Grasp Synthesis: } } We show preference percentages from users for each pairwise method comparison on HO3D and ObMAN. }
        \label{fig:user_study}
    \end{minipage}
    % Optionally, you can remove the joint caption if you have separate captions
    % \vspace{-2em}
\end{figure*}



% -----------

% \begin{figure}[ht]
%     \centering

%     \begin{minipage}{\linewidth}
%         \centering
%         \begin{center}
% \caption{\textbf{Comparison with Baselines:} We compare human grasp synthesis along with prior work~\cite{jiang2021hand} and annotated grasps provided by datasets(GT) on HO3D and ObMan. We report in table the amount of intersection between meshes, displacement distance in simulation, and hand contact ratio and area.  We also report preference percentages from users for pairwise method comparison on HO3D and ObMAN. }
% \vspace{-1em}

% \label{tab:grasp}

% % \vspace{-1em}
% \setlength{\tabcolsep}{2pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l c c c c c c c c c }
% \toprule

% % CATEGORIES
% &
% & \multicolumn{3}{c}{Intersection} 
% & \multicolumn{1}{c}{Disp.}
% & \multicolumn{2}{c}{Contact}
% \\
% % RULES
% \cmidrule(lr){3-5} \cmidrule(lr){6-6} \cmidrule(lr){7-8}

% & & maxD$\downarrow$  & avgD$\downarrow$ & vol$\downarrow$ & avg $\downarrow$  & ratio$\uparrow$ & area$\uparrow$ \\
% \midrule
% \multirow{3}{*}{HO3D} 
% & GT &  \textbf{1.32} &  0.37 &  6.16 &  2.32 & 0.95 & 0.15 \\
% & GraspTTA & 2.44 & 0.61 &  \textbf{5.25} & 2.89 &  1.00 &  0.23 \\
% & \ours &  1.84 &  \textbf{0.31} & 11.46 &  \textbf{0.95} &  \textbf{1.00} &  \textbf{0.23} \\

% \midrule

% \multirow{3}{*}{ObMan} 
% & GT & 0.98 & 0.74 &  \textbf{1.70} &  1.57 &  1.00 & 0.12 \\
% & GraspTTA &  0.87 &  0.58 &  5.56 &  \textbf{1.54} &  \textbf{1.00} &  0.18 \\
% & \ours &  \textbf{0.74} &  \textbf{0.51} & 17.40 & 1.85 & 0.93 &  \textbf{0.25} \\


% \bottomrule
% \end{tabular}
% }

% \end{center}

%     \end{minipage}\hfill

%     \begin{minipage}{\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{fig/userstudy.pdf}
%         %\caption{Figure caption} % uncomment if you want a separate caption for the figure
%     \end{minipage}\hfill
    
%     % \caption{Joint caption for both the figure and table.}
%     \vspace{-2em}
% \end{figure}


==> table/grasp_old.tex <==


\begin{figure}[ht]
    \centering

    \begin{minipage}{\linewidth}
        \centering
        \begin{center}
\captionof{table}{\textbf{Comparison with Baselines:} We compare our synthesised human grasps against GraspTTA~\cite{jiang2021hand} and annotated grasps provided by datasets(GT) on HO3D and ObMan. We report table the intersection between meshes, displacement distance in simulation, and hand contact ratio and area  (top).  We also report preference percentages from users for pairwise method comparison on HO3D and ObMAN (bottom). }
\vspace{-1em}

\label{tab:grasp}

% \vspace{-1em}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l l c c c c c c c c }
\toprule

% CATEGORIES
&
& \multicolumn{3}{c}{Intersection} 
& \multicolumn{1}{c}{Disp.}
& \multicolumn{2}{c}{Contact}
\\
% RULES
\cmidrule(lr){3-5} \cmidrule(lr){6-6} \cmidrule(lr){7-8}

& & maxD$\downarrow$  & avgD$\downarrow$ & vol$\downarrow$ & avg $\downarrow$  & ratio$\uparrow$ & area$\uparrow$ \\
\midrule
\multirow{3}{*}{\rotatebox{90}{HO3D}}
& GT &  \textbf{1.32} &  0.37 &  6.16 &  2.32 & 0.95 & 0.15 \\
& GraspTTA & 2.44 & 0.61 &  \textbf{5.25} & 2.89 &  1.00 &  0.23 \\
& \ours &  1.84 &  \textbf{0.31} & 11.46 &  \textbf{0.95} &  \textbf{1.00} &  \textbf{0.23} \\

\midrule

\multirow{3}{*}{\rotatebox{90}{ObMan}} 
& GT & 0.98 & 0.74 &  \textbf{1.70} &  1.57 &  1.00 & 0.12 \\
& GraspTTA &  0.87 &  0.58 &  5.56 &  \textbf{1.54} &  \textbf{1.00} &  0.18 \\
& \ours &  \textbf{0.74} &  \textbf{0.51} & 17.40 & 1.85 & 0.93 &  \textbf{0.25} \\


\bottomrule
\end{tabular}
}

\end{center}
    \vspace{0.5em}
    \end{minipage}\hfill

    \begin{minipage}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/userstudy.pdf}
        %\caption{Figure caption} % uncomment if you want a separate caption for the figure
    \end{minipage}\hfill
    
    % \caption{Joint caption for both the figure and table.}
    \vspace{-2em}
\end{figure}


==> table/improve.tex <==


%------------------------------------------------------------------------

% \definecolor{first}{rgb}{1.0, .79, 0.156}
\definecolor{first}{rgb}{1.0, .83, 0.3}
\definecolor{second}{rgb}{1.0, 0.93, 0.7}
% \definecolor{second}{rgb}{1.0, 0.88, 0.51}
% \definecolor{third}{rgb}{1.0, 0.93, 0.7}
\def \first {\cellcolor{first}}
\def \second {\cellcolor{second}}
% \def \third {\cellcolor{third}}
\def \third {}

\begin{table}[t]
\footnotesize
\begin{center}
\caption{\textbf{Improving Single-View Reconstruction} }
\label{tab:prior_obj}

% \vspace{-1em}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l c c c c c c c}
\toprule

% CATEGORIES
& \multicolumn{3}{c}{Object Error} 
& \multicolumn{1}{c}{Align}
& \multicolumn{2}{c}{Hand Error} \\

% RULES
\cmidrule(r){2-4} \cmidrule(r){5-5} \cmidrule(r){6-7} 


& $F@5$  & $F@10$ & $CD$  & $CD_h$ & MPJPE & AUC \\
\midrule

% NUMBERS
iHOI on HOI4D & \first \textbf{0.76} & \first \textbf{0.97} & \first \textbf{0.4} & \first \textbf{18.4} & \first \textbf{1.05} & \first 0.79 \\
method1+\ours \\
\midrule
\todo{AlignSDF on HO3D?} \\
\todo{method2+\ours} \\
\bottomrule
\end{tabular}
}

\end{center}
\end{table}


==> table/recon_ablation.tex <==


%------------------------------------------------------------------------

% \definecolor{}{rgb}{1.0, .79, 0.156}
% \definecolor{}{rgb}{1.0, .83, 0.3}
% \definecolor{}{rgb}{1.0, 0.93, 0.7}
% \definecolor{}{rgb}{1.0, 0.88, 0.51}
% \definecolor{third}{rgb}{1.0, 0.93, 0.7}
% \def \ {\cellcolor{}}
% \def \ {\cellcolor{}}
% \def \third {\cellcolor{third}}
% \def \third {}

\begin{table}[t]
\footnotesize
\begin{center}
\vspace{-1em}
\caption{\textbf{Ablation Study: } We ablate if reconstruction benefits from priors in the 3D space or from joint modeling hand and object. We also analyze the effect of adaptive SDS noise. }
\label{tab:ablate_recon}
\vspace{-1em}
% \vspace{-1em}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l c c c c c c c}
\toprule

% CATEGORIES
& \multicolumn{3}{c}{Object Error} 
& \multicolumn{1}{c}{Align}
& \multicolumn{2}{c}{Hand Error} \\

% RULES
\cmidrule(r){2-4} \cmidrule(r){5-5} \cmidrule(r){6-7} 


& F5$\uparrow$  & F10$\uparrow$ & CD$\downarrow$  & CD$_h$ $\downarrow$ & MPJPE$\downarrow$ & AUC$\uparrow$ \\
\midrule

% NUMBERS
\ours & \textbf{0.76} & \textbf{0.97} & \textbf{0.4} & \textbf{18.4} & \ 1.05 & \ 0.79 \\
Conditional & 0.66 & 0.92 & 0.7 & \ 19.3 & 1.14 & 0.77 \\
const-0.25 & \ 0.69 & \ 0.95 & \ 0.5 & 50.0 & \ \textbf{1.01} & \ \textbf{0.80} \\
const-0.75 & 0.49 & 0.76 & 4.0 & 48.1 & 1.06 & 0.79 \\
\bottomrule
\end{tabular}
}

\end{center}
\end{table}

